Efficient Sequential Calibration with $O(T^{2/3-\epsilon})$ Error Bound

We study the online binary sequential calibration problem. A recent breakthrough by \citet{dagan2024breaking} overcomes the classical \(T^{2/3}\) barrier for calibration error. Building on this result, we present an efficient randomized forecaster that achieves an expected calibration error \(O(T^{2/3-\varepsilon})\) for some constant \(\varepsilon>0\). Our forecaster combines the \textsc{SPR-Calibration} procedure \citep{dagan2024breaking} with an outer Blackwell-style correction layer. The \textsc{SPR-Calibration} procedure controls calibration with respect to a surrogate sequence of conditional-mean estimates, while the correction layer controls the additional error incurred when these surrogates are used to approximate the true outcomes. The analysis decomposes the total calibration error into the surrogate calibration error and the residual discrepancy between the surrogate sequence and the true outcomes. The former is bounded by the \textsc{SPR-Calibration} guarantee in \citet{dagan2024breaking}, and the latter is controlled using a quadratic potential argument together with the sparsity of the \textsc{SPR-Calibration} forecaster.

==> time_cost.tex <==


\subsection{Computational cost of Algorithm~\ref{alg:main}}

Recall that $|\mathcal{X}| = O(1/\eta) = O(\sqrt{T})$ and $\tau = \log_2(T)$.
We analyze the running time of Algorithm~\ref{alg:main} over \(T\) rounds.
The time cost has three components:
\begin{itemize}
    \item Computing the read-only map \(D_t(x)\) for all
\(x\in\mathcal X\);
\item Solving the finite minimax program \eqref{eq:opt};
\item Running a \textsc{SPR-Calibration} instance.
\end{itemize}



\paragraph{Computing \(D_t(x)\) for all \(x\in\mathcal X\).}
Line~4 of Algorithm~\ref{alg:main} computes
\[
D_t(x)
=
\text{the forecast that \textsc{SPR-Calibration} would output from state }
S_t^{\mathrm{SPR}}
\text{ if its input were }x
\]
for every \(x\in\mathcal X\). Since each preview costs
\(O(\tau h\log T+C_{\mathrm{spr}}(T))\), computing all values
\(\{D_t(x):x\in\mathcal X\}\) costs
\[
O\!\left(M(\tau h\log T+C_{\mathrm{spr}}(T))\right)
\]
per round. In the polylogarithmic SPR-response case, this becomes
\[
O(M\tau h\log T)=O(Mh\log^2 T).
\]
If \(h=O(\log T)\), this is \(O(M\log^3 T)\).

\paragraph{Computing the residual labels \(\widehat R_{x,t-1}\).}
Store the external residuals \(R_{p,t}\) in a hash table indexed by the
numerical prediction value \(p\). Then for each \(x\in\mathcal X\), after
\(D_t(x)\) has been computed, the value
\[
\widehat R_{x,t-1}
=
\begin{cases}
R_{D_t(x),t-1}, & D_t(x)\in\mathcal P_{t-1},\\
0, & D_t(x)\notin\mathcal P_{t-1}
\end{cases}
\]
can be computed in expected \(O(1)\) time. Hence this line costs \(O(M)\) per
round.

\paragraph{Solving the finite minimax program.}
Let
\[
a_x:=\widehat R_{x,t-1}(0-x),
\qquad
b_x:=\widehat R_{x,t-1}(1-x).
\]
The minimax program is
\[
\min_{\mu\in\Delta(\mathcal X)}
\max
\left\{
\sum_{x\in\mathcal X}\mu(x)a_x,
\sum_{x\in\mathcal X}\mu(x)b_x
\right\}.
\]
Equivalently, one chooses a point in the convex hull of
\(\{(a_x,b_x):x\in\mathcal X\}\subseteq\mathbb R^2\) minimizing the maximum
coordinate. A simple implementation enumerating pairs of grid points solves
this problem in \(O(M^2)\) time per round. A convex-hull implementation solves
it in \(O(M\log M)\) time per round. We will use the conservative bound
\[
O(M^2)
\]
unless otherwise stated.

\paragraph{Running a \textsc{SPR-Calibration} instance.}
Sampling \(\widetilde e_t\sim\mu_t\) costs \(O(M)\) time if a cumulative
distribution is built explicitly. After sampling, the algorithm performs one
actual \textsc{SPR-Calibration} update using input \(\widetilde e_t\). This
costs
\[
O(\tau h\log T+C_{\mathrm{spr}}(T))
\]
time under the same data structures. If a committed SPR move deletes many
signs, the deletions can be charged amortized: each sign is inserted at most
once before it is deleted, so the total number of committed sign deletions
over all rounds is at most the total number of committed sign insertions,
which is at most \(T\). Including segment-tree updates, committed deletions
contribute at most \(O(T\log T)\) additional time over the whole run.

\paragraph{Residual bookkeeping.}
Membership testing for \(p_t\in\mathcal P_{t-1}\) and updating
\(R_{p_t,t}\) are hash-table operations and cost expected \(O(1)\) time. The
line
\[
R_{p,t}\gets R_{p,t-1}
\qquad
\text{for all }p\in\mathcal P_t\setminus\{p_t\}
\]
should be implemented lazily: residuals that do not change are simply left
untouched. Thus this line costs \(O(1)\), not \(O(|\mathcal P_t|)\).






\begin{lemma}
The total running time of Algorithm~\ref{alg:main} is $O(T^2\log^3(T))$.
\end{lemma}
\begin{proof}
By the analysis above, the total time cost is bounded by
\[
O\!\left(
T^{\frac{3}{2}}(\tau h\log T+C_{\mathrm{spr}}(T))
+
T^2
+
T\log T
\right),
\]
where the \(T\log T\) term accounts for amortized committed sign deletions.
Under a polylogarithmic-time SPR response implementation, this simplifies to $
O\!\left(
T M\tau h\log T
+
T M^2
\right)
=
O\!\left(
T M h\log^2T
+
T M^2
\right)$. 
Noting that  \(h=O(\log T)\), the bound becomes $
O\!\left(
T M\log^3T
+
T M^2
\right)\leq O(T^2\log^3(T))$.
\end{proof}





The inner \textsc{SPR-Calibration} algorithm maintains SPR instances
\(G_{i,j,\ell}\), where \(i\le \tau\), \(j\in\{i+1,\ldots,i+h\}\), and
\(\ell\in\{0,1\}\). For a fixed level \(i\), each such instance has at most \(2^i\)
cells. Hence the total number of latent cells across all instances is
\[
\sum_{i=1}^{\tau} O(h\,2^i)=O(hT).
\]
Thus a fully explicit representation of all cell biases and signs requires
\(O(hT)\) space. Since \(h\le \tau=O(\log T)\), this is \(O(T\log T)\) space
in the usual parameter range.


For each SPR instance \(G\), store the cell biases in a segment tree. The
tree supports the following operations in \(O(\log T)\) time:
\[
\min_{\bar c<c}\operatorname{bias}(\bar c,G),
\qquad
\max_{\bar c>c}\operatorname{bias}(\bar c,G),
\]
as well as point updates to cell biases. Therefore, for a fixed candidate
surrogate \(x\), testing whether a given account admits removable bias costs
\(O(\log T)\). Since \textsc{SPR-Calibration} checks
\(O(\tau h)\) accounts in its priority order, the cost of previewing one
candidate \(x\) is
\[
O(\tau h\log T + C_{\mathrm{spr}}(T)),
\]
where \(C_{\mathrm{spr}}(T)\) denotes the time needed to compute the response
of the chosen SPR strategy when a new sign must be placed. If the SPR
response strategy is explicit and polylogarithmic-time, then
\(C_{\mathrm{spr}}(T)=\operatorname{polylog}(T)\), and this term is dominated
by the \(O(\tau h\log T)\) scan.

Thus, under a polylogarithmic-time SPR response implementation, one preview
costs
\[
O(\tau h\log T)=O(h\log^2 T).
\]
If \(h=O(\log T)\), this is \(O(\log^3 T)\).




\paragraph{Cost of committing one \textsc{SPR-Calibration} }
Indeed, \textsc{SPR-Calibration} checks the accounts \(G_{i,j,\ell}\) in its
priority order, where \(i\le \tau:=\lceil \log_2 T\rceil\),
\(j\in\{i+1,\ldots,i+h\}\), and \(\ell\in\{0,1\}\). For a fixed level \(i\),
each SPR instance has \(2^i\) cells. Without a range-query data structure,
checking whether there is removable negative bias to the left of the current
cell or removable positive bias to the right requires scanning the cells of
the relevant instance, which costs \(O(2^i)\). Therefore one full scan over
all relevant accounts costs
\[
\sum_{i=1}^{\tau} O(h\,2^i)=O(hT).
\]
The algorithm has a bias-removal pass and, if no removable bias is found, a
bias-placement pass. This changes only the constant factor. If
\texttt{simulateGame} is called, then deleting all legally removable signs in
the chosen instance can also be implemented by scanning that instance, which
costs \(O(2^i)\le O(T)\), and is dominated by the \(O(hT)\) scan. Hence the
committed inner update costs
\[
O(hT)
\]
time per round, and over \(T\) rounds the committed inner updates cost
\[
O(hT^2).
\]
If \(h=O(\log T)\), this contribution is \(O(T^2\log T)\).

If the preview computations \(D_t(x)\) are still implemented with range-query
data structures, while only the committed update is implemented naively, then
the total running time over \(T\) rounds is
\[
O\!\left(
T M h\log^2 T
+
T M^2
+
hT^2
\right),
\]
where \(M:=|\mathcal X|\). Here \(T M h\log^2T\) is the cost of computing
\(D_t(x)\) for all \(x\in\mathcal X\), \(TM^2\) is the cost of solving the
finite minimax problem with a simple \(O(M^2)\) solver, and \(hT^2\) is the
cost of the naive committed \textsc{SPR-Calibration} updates.

If, in addition, the previews are also implemented naively, then previewing
one candidate \(x\) costs \(O(hT)\), so computing \(D_t(x)\) for all
\(x\in\mathcal X\) costs \(O(MhT)\) per round. In that fully naive
implementation, the total running time over \(T\) rounds is
\[
O\!\left(
MhT^2
+
TM^2
\right).
\]
For \(h=O(\log T)\), this becomes
\[
O\!\left(
MT^2\log T
+
TM^2
\right).
\]
